Resource-Constrained Adaptive Search for Sparse Multi-Class Targets with Varying Importance

In sparse target inference problems it has been shown that significant gains can be achieved by adaptive sensing using convex criteria. We generalize previous work on adaptive sensing to (a) include multiple classes of targets with different levels of importance and (b) accommodate multiple sensor models. New optimization policies are developed to allocate a limited resource budget to simultaneously locate, classify and estimate a sparse number of targets embedded in a large space. Upper and lower bounds on the performance of the proposed policies are derived by analyzing a baseline policy, which allocates resources uniformly across the scene, and an oracle policy which has a priori knowledge of the target locations/classes. These bounds quantify analytically the potential benefit of adaptive sensing as a function of target frequency and importance. Numerical results indicate that the proposed policies perform close to the oracle bound (<3dB) when signal quality is sufficiently high (e.g.~performance within 3 dB for SNR above 15 dB). Moreover, the proposed policies improve on previous policies in terms of reducing estimation error, reducing misclassification probability, and increasing expected return. To account for sensors with different levels of agility, three sensor models are considered: global adaptive (GA), which can allocate different amounts of resource to each location in the space; global uniform (GU), which can allocate resources uniformly across the scene; and local adaptive (LA), which can allocate fixed units to a subset of locations. Policies that use a mixture of GU and LA sensors are shown to perform similarly to those that use GA sensors while being more easily implementable.

==> s_app_full_oracle_derivation_general.tex <==
\section{Derivation of (\ref{eq:oracle-allocation})}
\label{app:full-oracle-deriv-general}

From (\ref{eq:index-permutation-definition}), we can easily see that
\begin{equation}
\label{eq:h-pi-ordering-oracle}
h(C_{\pi(i)}) = \begin{cases}
h(|\calC|), & i=1,2,\dots,N_{|\calC|}\\
h(|\calC|-1), & i=N_{|\calC|}+1,\dots,N_{|\calC|}+N_{|\calC|-1}\\
\vdots, &\vdots\\
h(2), & i=N-N_1-N_2+1,\dots,N-N_1\\
h(1)=0, & i=N-N_1+1,\dots,N
\end{cases}
\end{equation}
Inspecting \eqref{eq:h-pi-ordering-oracle} further, we note an important property in the case where $C_{\pi(i)}\neq C_{\pi(i+1)}$. Specifically, we have
\begin{equation}
\label{eq:d-pi-def}
\pi(i) = \sum\limits_{c=d}^{|\calC|} N_c
\end{equation}
for some $d\in\set{2,3,\dots,|\calC|}$.  Moreover, if $d$ is chosen to satisfy \eqref{eq:d-pi-def} and $N_c>0$ for all $c\in\calC$, then we have
\begin{equation}
\label{eq:hd-def}
\begin{split}
h(C_{\pi(i)}) &= h(d)\\
h(C_{\pi(i)+1}) &= h(d-1)
\end{split}
\end{equation}
We derive the optimal solution for the oracle policy by noting that minimizing the cost function in Lemma \ref{lemma:cost-determ-lambda} given an overall budget constraint $\sum_{i=1}^N \overline{\lambda_i} = \Lambda$ is of identical form to \eqref{eq:greedy-problem} by replacing $z_i(t)=h(C_i)$, $\sigma_i^2(t)=\sigma_0^2$, and $\lambda_i(t)=\overline{\lambda_i}$.  Thus, we have
\begin{equation}
\begin{split}
g(k) &= c_0 \left( \sum\limits_{i=1}^k \frac{\sqrt{h(C_{\pi(i)}})}{\sqrt{h(C_{\pi(k+1)}})} - k\right)
\end{split}
\end{equation}
There are two regimes of interest to further simplify this function: (a) when $C_{\pi(k+1)}=C_{\pi(k)}$ and (b) when $C_{\pi(k+1)}\neq C_{\pi(k)}$.  In the former case we note that
\begin{equation}
\label{eq:gk-sameclass}
\begin{split}
g(k) &= c_0\left(\sum\limits_{i=1}^k\frac{\sqrt{h(C_{\pi(i)})}}{\sqrt{h(C_{\pi(k)})}} - k\right)\\
&= c_0\left(\sum\limits_{i=1}^{k-1}\frac{\sqrt{h(C_{\pi(i)})}}{\sqrt{h(C_{\pi(k)})}} - (k-1)\right)= g(k-1)
\end{split}
\end{equation}
Therefore, within intervals where $C_{\pi(k)}=C_{\pi(k+1)}$, we have equal values of $g(k)$.  This implies that when there is sufficient budget to search for a single target of a given class, then we should search for all targets of that class.  When $C_{\pi(k+1)}\neq C_{\pi(k)}$, we note from \eqref{eq:d-pi-def} and \eqref{eq:hd-def} that
\begin{equation}
\label{eq:gk-diffclass}
\begin{split}
g(\pi(k)) &= c_0\left(\frac{1}{\sqrt{h(\tilde{d}(k)-1)}}\sum\limits_{i=1}^k\sqrt{h(C_{\pi(i)})}- \sum\limits_{c=\tilde{d}(k)}^{|\calC|} N_c\right)\\
&= c_0\left(\frac{1}{\sqrt{h(\tilde{d}(k)-1)}}\sum\limits_{c=\tilde{d}(k)}^{|\calC|}{N_c\sqrt{h(c)}}- \sum\limits_{c=\tilde{d}(k)}^{|\calC|} N_c\right)
\end{split}
\end{equation}
where
\begin{equation}
\label{eq:tilde-dk}
\tilde{d}(k) = \set{d\in\set{2,3,\dots,|\calC|}:  \sum\limits_{c=d}^{|\calC|} N_c \leq k < \sum\limits_{c=d-1}^{|\calC|} N_c}
\end{equation}
Using (\ref{eq:gk-sameclass}), (\ref{eq:gk-diffclass}), (\ref{eq:tilde-dk}), and noticing that $g(1)=0$, we have
\begin{equation}
g(k) = \begin{cases}
0, & k<N_{|\calC|},\\
\infty, &k \geq N-N_1\\
c_0\sum\limits_{c=\tilde{d}(k)}^{|\calC|}N_c\left(\dfrac{\sqrt{h(c)}}{\sqrt{h(\tilde{d}(k)-1)}}-1\right), &\mathrm{else}.
\end{cases}
\end{equation}
Note that $\tilde{d}(k)$ is constant for all targets of the same class, and thus so is $g(k)$.  The number of nonzero allocations $k^*$ is given by the interval where $\Lambda\in(g(k^*-1),g(k^*)]$.  We can conclude that when the oracle policy allocates any resources to a target with class $c$, then it must allocate to all targets with class $c$.  The oracle policy is then given by
\begin{equation}
{\overline{\lambda_{\pi(i)}^{o}}}=\begin{cases}
\dfrac{\left(\Lambda+k^*c_0\right)\sqrt{h(C_{\pi(i)})}}{\sum_{j=1}^{k^*}\sqrt{h(C_{\pi(j)})}}-c_0, & i=1,\dots,k^*\\
0, & \mathrm{else}\end{cases}
\end{equation}
We can simplify this further using Assumption \ref{ass:high-snr-assumption-oracle1} where we have
\begin{equation}
\begin{split}
\Lambda \geq c_0 \Lambda_0 &= c_0\sum\limits_{c=2}^{|\calC|} N_c\sqrt{\frac{h(c)}{h(2)}}-(N-N_1)\\
&= g(N-N_1-1)
\end{split}
\end{equation}
Since $g(N-N_1)=\infty$, we have $\Lambda \in (g(N-N_1-1),g(N-N_1)]$ so that $k^*=N-N_1$.  Plugging into \eqref{eq:oracle-allocation}, we have 
\begin{equation}
\begin{split}
\overline{\lambda_{\pi(i)}^o} &= \left(\Lambda+(N-N_1)c_0\right)\left(\dfrac{\sqrt{h(C_{i})}}{\sum_{c=2}^{|\calC|}N_c\sqrt{h(c)}}\right)-c_0
\end{split}
\end{equation}
for $C_i>1$ and zero else.


==> s_app_missP_general.tex <==
\section{Proposition 2}\label{app:missclassification-prob}
\begin{proof}
Given the observation history $\vY(t-1)$, the posterior distribution $\pic{c}(t)$ will only depend on $y_i(t)$. $\hat C_i(t)$ (defined in (\ref{equ:estimated-C})) is a function of $\pic{c}(t)$, therefore also only depends on $y_i(t)$. For brevity, $\vY(t-1)$ is left out in the following deductions. But it should be noticed all quantities are dependent on $\vY(t-1)$.

 Define $\bm c(t)$ as the set of $c$ that could possibly be $\hat C_i(t)$ for some $y_i(t)$:
\begin{align}
\bm c(t) = \{c|\hat C_i(t)=c \text{ for some } y_i(t)\}
\end{align}
 Define $\text{y}^{(c)}_i$ as the decision region that will lead to $\hat C_i(t)=c$:
\begin{align}\label{equ:y-interval}
\text{y}^{(c)}_i(t)=&\{y_i(t)\in\mathbb{R}|\hat C_i(t)=c\} %\notag \\
%	=&\{y_i(t)\in\mathbb{R}|c=\arg\max_{d\in\bm c(t)}~ \pic{d}(t)\} 
\end{align}

The probability distribution of $y_i(t)$ is given by (\ref{equ:y_t-prob}). Notice $y_i(t)$ share the same variance across target classes when $c>1$. Denote the variance for $c=1$ and $c>1$ respectively as:
\begin{align}\label{equ:y(t)}
\Sigma^0_i(t)=&\nu^2/\lambda_i(t-1)\notag \\
\Sigma_i(t)=& \sigma^2_i(t-1)+\nu^2/\lambda_i(t-1)
\end{align}

Denote $m_c = \hatXic{c}(t-1)$, and rank the elements in $\bm c(t)$ with sequence $\pi(c)$ such that:
\begin{align}
m_{\pi(1)}<m_{\pi(2)}<m_{\pi(3)}<\cdots
\end{align}

\begin{lemma}
$\text{y}^{(c)}_i(t)$ are simple intervals: 
\begin{align}
\cdots,~& (a_i^{\pi(-2)}(t),~a_i^{\pi(-1)}(t)],
~ (a_i^{\pi(-1)}(t), a_i^{0}(t)],\notag \\
& ~(a_i^{0}(t), a_i^{1}(t)],~(a_i^{1}(t), a_i^{\pi(1)}(t)],\cdots
\end{align}
\ignore{Further denote $m_c = \hatXic{c}(t-1)$, and class for each interval as $m_{\pi(c)}$,}
and the posterior probability at the boundary $a_i^{\pi(c)}(t)$ is the same for two adjacent classes:
\begin{align}\label{equ:equal-prob}
& \pic{\pi(c)}(t-1)f(a_i^{\pi(c)}|C_i=\pi(c)) \notag \\
=& \pic{\pi(c+1)}(t-1)f(a_i^{\pi(c)}|C_i=\pi(c+1))
\end{align}
\end{lemma}

\ifjournal
	\begin{proof}
	Proof will be provided in full length report.
	\end{proof}
	By definition (\ref{equ:missP-def}), 
	\begin{align}
	 q_i(t) =&\Pr\left(\hat{C}_i(t)\neq C_i|\vY(t-1)\right)\notag \\
	=& 1 - \tilde{q}_i(t)
	\end{align}
\else
	\input{s_app_missP_lemma}
	By definition (\ref{equ:missP-def}), 
	\begin{align}
	 q_i(t) =&\Pr\left(\hat{C}_i(t)\neq C_i|\vY(t-1)\right)\notag \\
	 \intertext{Notice $\Pr\left(\hat{C}_i(t)=c|\vY(t-1)\right)=0$ if $c\notin \bm c(t)$,}
	=& \sum_{c\in\bm c(t)}\pic{c}(t-1) \Pr\left(\hat C_i(t)\neq c\big|C_i=c,\vY(t-1)\right)\notag \\
	= & \sum_{c\in\bm c(t)}\pic{c}(t-1)\left(1-
	\int_{\text{y}^{(c)}_i(t)} f(y_i(t)|C_i=c) dy_i(t)\right) \notag\\
	=& 1- \sum_{c\in\bm c(t)}\pic{c}(t-1)\int_{\text{y}^{(c)}_i(t)} f(y_i(t)|C_i=c) dy_i(t) \notag \\
	=& 1 - \tilde{q}_i(t)
	\end{align}
\fi	

Where 
\begin{align}\label{equ:correct_class}
\tilde{q}_i(t)= \sum_{c\in\bm c(t)}\pic{c}(t-1)\int_{\text{y}^{(c)}_i(t)} f(y_i(t)|C_i=c) dy_i(t)
\end{align}
is the probability of correct classification.

Denote $\Phi()$ as standard normal cumulative probability function, $\Phi'()$ as the standard normal probability density function. Further define normalized boundaries of $\text{y}^{\pi(c)}_i(t)$:
{\footnotesize \begin{align}
&  b^{1}_l = \frac{a^{0}_i(t)}{\sqrt{\Sigma^0_i(t)}}, \quad b^{1}_r = \frac{a^{1}_i(t)}{\sqrt{\Sigma^0_i(t)}} \notag \\
& b^{\pi(d)}_l= \frac{a^{\pi(d)}_i(t)-m_{\pi(d)}}{\sqrt{\Sigma_i(t)}}, \quad
b^{\pi(d)}_r = \frac{a^{\pi(d+1)}_i(t)-m_{\pi(d)}}{\sqrt{\Sigma_i(t)}}. 
\end{align}}
Then
{\footnotesize  \begin{align}
\tilde{q}_i(t)=&\sum_{c\in\bm c(t)}\pic{c}(t-1)\int_{\text{y}^{(c)}_i(t)} f(y_i(t)|C_i=c) dy_i(t) \notag \\
=& \sum_{k\leq -1}\pic{\pi(k)}(t-1)\left( \Phi(b^{\pi(k)}_r)-\Phi(b^{\pi(k)}_l)\right) \notag \\
 & +\pic{1}(t-1)\left( \Phi(b^{1}_r)-\Phi(b^{1}_l)\right) \notag \\
& +\sum_{k\geq 1}\pic{\pi(k)}(t-1)\left( \Phi(b^{\pi(k)}_r)-\Phi(b^{\pi(k)}_l)\right) \notag \\
\intertext{break the summation and rearrange terms}
=& \pic{\pi(-1)}(t-1)\Phi(b^{\pi(-1)}_r) - \pic{1}(t-1)\Phi(b^{1}_l)+ \notag \\
& \pic{1}(t-1)\Phi(b^{1}_r) - \pic{\pi(1)}(t-1)\Phi(b^{\pi(1)}_l)+ \notag \\
&\sum_{k\geq 1,k<-1}\pic{\pi(k)}(t-1) \Phi(b_r^{\pi(k)})-\pic{\pi(k+1)}(t-1)\Phi(b^{\pi(k+1)}_l) \notag \\
=& M^{1,l}_i(t) + M^{1,r}_i(t) + \sum_{k>1,k<-1} M^k_i(t)
\end{align}}

$b^{\pi(k)}_l$,$b^{\pi(k)}_r$ are functions of $a_i^{\pi(c)}(t)$, $a_i^{\pi(c)}(t)$ is function of $\Sigma_i(t)$ and $\Sigma^0_i(t)$, $\Sigma_i(t)=\Sigma^0_i(t)+\sigma_i^2(t)$. Therefore, $M^k_i(t)$ depends on $\lambda_i(t)$ through $\Sigma^0_i(t)$.

{\footnotesize \begin{align}
& \frac{d M^{1,l}_i(t)}{d \Sigma_i^0(t)} \notag \\
= &\pic{\pi(-1)}(t-1) \Phi'(b^{\pi(-1)}_r) \left(-\frac{b^{\pi(-1)}_r}{2\Sigma_i(t)} +\frac{1}{\sqrt{\Sigma_i(t)}}\frac{d a^{0}_i(t)}{d\Sigma^0_i(t)}\right) \notag \\
& -  \pic{1}(t-1) \Phi'(b^{1}_l) \left(-\frac{b^{1}_l}{2\Sigma^0_i(t)}+ \frac{1}{\sqrt{\Sigma^0_i(t)}}\frac{d a^{1}_i(t)}{d\Sigma^0_i(t)}\right) \notag \\
%=& \pic{\pi(-1)}(t-1) f(a^{0}_i(t)|\pi(-1)) \left(-\frac{b^{\pi(-1)}_r}{2\sqrt{\Sigma_i(t)}} +\frac{d a^{0}_i(t)}{d\Sigma^0_i(t)}\right) \notag \\
%& - \pic{1}(t-1)f(a^{0}_i(t)|1)\left( -\frac{b^{1}_l}{2\sqrt{\Sigma^0_i(t)}}+ \frac{d a^{0}_i(t)}{d\Sigma^0_i(t)} \right) \notag \\
\intertext{Plug in  $\Phi'(b^{\pi(-1)}_l)/\sqrt{\Sigma_i(t)}= f(a^{0}_i(t)|\pi(-1))$,  $ \Phi'(b^{1}_l)/\sqrt{\Sigma^0_i(t)}= f(a^{0}_i(t)|1)$ and (\ref{equ:equal-prob}),}
=& -\pic{\pi(1)}(t-1) f(a^{0}_i(t)|1) \frac{\sqrt{A_{\pi(-1)}}}{2\Sigma^0_i(t)\Sigma_i(t)} 
\leq 0
\end{align}}

Similarly
{\footnotesize \begin{align}
 \frac{d M^{1,r}_i(t)}{d \Sigma_i^0(t)} = -\pic{1}(t-1) f(a^{1}_i(t)|1) \frac{\sqrt{A_{\pi(1)}}}{2\Sigma^0_i(t)\Sigma_i(t)} \leq 0
\end{align}}

When $k\geq 1$ or $k<-1$,
{\footnotesize\begin{align}
& \frac{dM^k_i(t)}{d\Sigma^0_i(t)} \notag \\
=& \pic{\pi(k)}(t-1)\Phi'(b^{\pi(k)}_r)
\left(-\frac{b^{\pi(k)}_r}{2\Sigma_i(t)}+\frac{1}{\sqrt{\Sigma_i(t)}}\frac{da^{\pi(k)}_i(t)}{d\Sigma^0_i(t)}\right) \notag \\
& -\pic{\pi(k+1)}(t-1)\Phi'(b^{\pi(k+1)}_l)
\left(-\frac{b^{\pi(k+1)}_l}{2\Sigma_i(t)}+\frac{1}{\sqrt{\Sigma_i(t)}}\frac{da^{\pi(k)}_i(t)}{d\Sigma^0_i(t)}\right) \notag\\
%=& \pic{\pi(k)}(t-1)f(a^{\pi(k)}_i(t)|\pi(k))
%\left(-\frac{b^{\pi(k)}_r}{2\sqrt{\Sigma_i(t)}}+\frac{da^{\pi(k)}_i(t)}{d\Sigma^0_i(t)}\right) \notag \\
%& -\pic{\pi(k+1)}(t-1)f(a^{\pi(k)}_i(t)|\pi(k+1))
%\left(-\frac{b^{\pi(k+1)}_l}{2\Sigma_i(t)}+\frac{da^{\pi(k)}_i(t)}{d\Sigma^0_i(t)}\right) \notag\\
%\intertext{Plug in (\ref{equ:equal-prob})}
= & \pic{\pi(k)}(t-1)f(a^{\pi(k)}_i(t)|\pi(k))\frac{m_{\pi(k)}-m_{\pi(k+1)}}{2\Sigma_i(t)} 
\leq 0
\end{align}}
Therefore,
\begin{align}
\frac{d\tilde{q}_i(t)}{d\Sigma^0_i(t)} \leq 0
\end{align}
Further from  (\ref{equ:y(t)}), $\frac{d\Sigma^0_i(t)}{d\lambda_i(t)}<0$, therefore
\begin{align}
\frac{d\tilde{q}_i(t)}{d\lambda_i(t)}\geq 0, \qquad \frac{dq_i(t)}{d\lambda_i(t)}\leq 0
\end{align}
\end{proof}


==> s_app_missP_lemma_general.tex <==
\begin{proof}
First compare the posterior probability when $c\neq 1$:
\begin{align}
& \arg\max_{d\in\bm c(t),d\neq 1} \pic{d}(t) \notag \\
\intertext{plug in (\ref{eq:prob-update}) and ignore the constant in denominitor}
=& \arg\max_{d\in\bm c(t),d\neq 1} \pic{d}(t-1) f(y_i(t)|C_i=c) \notag \\
\intertext{plug in (\ref{equ:y_t-prob}) and formula for normal distribution}
=& \arg\max_{d\in\bm c(t),d\neq 1} \frac{\pic{d}(t-1)}{ \sqrt{\Sigma_i(t)}}
 \exp\left\{ -\frac{(y_i(t)-m_d)^2}{ 2\Sigma_i(t)} \right\} \notag \\
\intertext{take logrithm}
=& \arg\max_{d\in\bm c(t),d\neq 1} \left(\log\frac{\pic{d}(t-1)}{ \sqrt{\Sigma_i(t)}}
  -\frac{(y_i(t)-m_d)^2}{ 2\Sigma_i(t)} \right) \notag \\
\intertext{change max to min, and ignore constant $\log\sqrt{\Sigma_i(t)}$}
=& \arg\min_{d\in\bm c(t),d\neq 1} \left( \frac{(y_i(t)-m_d)^2}{2\Sigma_i(t)} -\log \pic{d}(t-1)  \right)
\end{align}
The functions within the minimization are quadratic in $y_i(t)$, and have the same shapes across classes $d$. Therefore, the minimum, i.e. $\text{y}^{(c)}_i(t)$, are simple intervals, and equation (\ref{equ:equal-prob}) holds.

Now consider the case $\hat C_i(t)=1$.
\begin{align}
& \hat C_i(t) = 1 \notag \\
\leftrightarrow~ & 1 = \arg\max_{d\in\bm c(t)} \pic{d}(t) \notag \\
\leftrightarrow~ &  \pic{1}(t)  \geq \pic{d}(t)\quad \forall d\in \bm c(t) \notag \\
\leftrightarrow~ & \pic{1}(t-1)f(y_i(t)|C_i=1)\geq \pic{d}(t-1)f(y_i(t)|C_i=d)  \notag \\
\intertext{plug in (\ref{equ:y_t-prob}) }
\leftrightarrow~ & \pic{1}(t-1) \frac{\exp\left\{ -\frac{y_i(t)^2}{ 2\Sigma^0_i(t)}\right\}}{\sqrt{2\pi\Sigma^0_i(t)}} \geq \pic{d}(t-1)\frac{\exp\left\{ -\frac{(y_i(t)-m_d)^2}{ 2\Sigma_i(t)}\right\}}{\sqrt{2\pi\Sigma_i(t)}} \notag \\
\leftrightarrow~ & \frac{\pic{1}(t-1)}{\pic{d}(t-1))}\geq
\sqrt{\frac{\Sigma^0_i(t)}{\Sigma_i(t)}} \exp\left\{ \frac{y_i(t)^2}{ 2\Sigma^0_i(t)} -\frac{(y_i(t)-m_d)^2}{2\Sigma_i(t)}\right\} \notag \\
\intertext{take logrithm}
\leftrightarrow~ & \frac{\sigma_i^2(t)}{2\Sigma^0_i(t)\Sigma_i(t)}y_i(t)^2 +\frac{m_d}{\Sigma_i(t)}y_i(t) -\frac{\mu_d^2}{2\Sigma_i(t)} \notag \\
& \leq \frac{1}{2}\log\frac{\Sigma_i(t)}{\Sigma^0_i(t)} + \log\frac{\pic{1}(t-1)}{\pic{d}(t-1)} \quad \forall d\in \bm c(t) \notag
\end{align}

Solve above inequality and recall the definition in (\ref{equ:estimated-C}):
\begin{align}
\text{y}^{(1)}_i(t) = (-\infty, a^{\pi(1)}_i(t)]
\end{align}
where
\begin{align}
& a^{\pi(1)}_i(t) =
 \left\{ \begin{array}{ll}
0 & \text{if }  A\leq 0 \\
-\frac{\Sigma^0_i(t)m_{\pi(2)}}{\sigma^2_i(t)}+\sqrt{A} & \text{if $A\geq 0$ } 
\end{array} \right. \notag \\
& A = \frac{\Sigma_i(t)\Sigma_i^0(t)}{\sigma^2_i(t)}
\left(\frac{m^2_{\pi(2)}}{\sigma^2_i(t)} -2\log\frac{\pic{\pi(2)}(t-1)}{\pic{1}(t-1)}+\log\frac{\Sigma_i(t)}{\Sigma_i^0(t)}\right) \notag
\end{align}
\ignore{\begin{align}
\text{y}^{(1)}_i(t) =& \left\{ \begin{array}{ll}
\emptyset & \text{if }  A_d\leq 0~\forall d \\
(a_i^{0}(t),a^1_i(t)] & \text{otherwise }
\end{array} \right. 
\end{align}
where
\begin{align}
A_d = & \frac{\Sigma_i(t)\Sigma_i^0(t)}{\sigma^2_i(t)}
\left(\frac{m^2_d}{\sigma^2_i(t)} -2\log\frac{\pic{d}(t-1)}{\pic{1}(t-1)}+\log\frac{\Sigma_i(t)}{\Sigma_i^0(t)}\right) \notag \\
a_i^{0}(t) = & -\frac{\Sigma_i^0(t)m_{\pi(-1)}}{\sigma^2_i(t)}-\sqrt{A_{\pi(-1)}} \notag \\
a_i^{1}(t) = & -\frac{\Sigma_i^0(t)m_{\pi(1)}}{\sigma^2_i(t)}+\sqrt{A_{\pi(1)}} \notag
\end{align}
It should be noticed that it is possible that the two intervals on the left and right of class 1 are from the same target class, $\pi(-1)=\pi(1)$. However, it does not affect our result.

If $\text{y}^{1}_i(t)=\emptyset$, the miss-classification problem is straight-forward, therefore we only consider the case that  $\text{y}^{1}_i(t)\neq \emptyset$, i.e. $1\in\bm c(t)$. In this case, the posterior probability at $a_i^{0}$ is the same for class $\pi(-1)$ and 1, and posterior probability at $a_i^{1}$ is the same for class 1 and $\pi(1)$:
\begin{align}\label{equ:a_1}
& \pic{\pi(-1)}(t-1)f(a_i^{0}|\pi(-1))= \pic{1}(t-1)f(a_i^{0}|1) \notag \\
& \pic{1}(t-1)f(a_i^1|1)= \pic{\pi(1)}(t-1)f(a_i^1|\pi(1))
\end{align}}
When $A<0$, the problem becomes misclassification problem over class 1 targets is 0.5, and the problem becomes trivial. Here we consider the case $A\geq 0$, in which case Equation (\ref{equ:equal-prob}) also holds.

To sum up two cases,  Equation (\ref{equ:equal-prob}) holds.
\end{proof}
